NVMExplorer: A Framework for Cross-Stack Comparisons of Embedded Non-Volatile Memories

Repeated off-chip memory accesses to DRAM drive up operating power for data-intensive applications, and SRAM technology scaling and leakage power limits the efficiency of embedded memories. Future on-chip storage will need higher density and energy efficiency, and the actively expanding field of emerging, embeddable non-volatile memory (eNVM) technologies is providing many potential candidates to satisfy this need. Each technology proposal presents distinct trade-offs in terms of density, read, write, and reliability characteristics, and we present a comprehensive framework for navigating and quantifying these design trade-offs alongside realistic system constraints and application-level impacts. This work evaluates eNVM-based storage for a range of application and system contexts including machine learning on the edge, graph analytics, and general purpose cache hierarchy, in addition to describing a freely available (http://nvmexplorer.seas.harvard.edu/) set of tools for application experts, system designers, and device experts to better understand, compare, and quantify the next generation of embedded memory solutions.

==> arch_driven_opps.tex <==
%\subsection{Architecture-Driven Opportunities} \label{subsec:arch_driven}

%Despite the reliance of architects on device designers (with respect to which memory technologies are available), 
There are many opportunities for architects to innovate alongside device designers in order to best take advantage of the current eNVM technology proposals available. In fact, \NAME~can be used to analytically probe architectural opportunities to best leverage the unique trade-offs of eNVM devices compared to more traditional devices. Examples of these critical system-level choices include intermittent operation (Section \ref{subsubsec:intermittent}) and write buffering (Section \ref{subsubsec:write-buf}). 

%, and an alternative level in the memory hierarchy (Section \ref{subsec:new-mem-level}).

%\textcolor{red}{fixme; Reiterate caveats and/or limitations and what future versions can/will be expanded to do?}

\subsection{Intermittent Operation Highlights Relative\\ eNVM Benefits} 
\label{subsec:intermittent}

As demonstrated in the domain-specific case of DNN inference under continuous vs. intermittent operation in Section \ref{subsec:dnn}, non-volatility of on-chip storage resources is a particularly compelling property for resource-constrained systems that experience intermittent power supply (e.g., deployed solar-powered agricultural sensors or satellites) or otherwise operate intermittently (e.g., a voice-enabled assistant executing NLP tasks on wake-up). Across a range of potential device wake-up frequency and per-wake-up compute patterns, we can make the high-level observation that several eNVM proposals become particularly compelling under these conditions, and the preferred NVM choice for further investigation varies depending on both of these factors. Figure~\ref{fig:intermittent} shows total energy as a function of inference per day for two workloads of interest: ResNet26 (image classification) and ALBERT (NLP). Here total energy is presented because it is the closest proxy we have for battery life. From the figure, we can observe that when the number of inferences per day is sufficiently low (less than 1e5 for ResNet and less than 1e4 for ALBERT), the opt. FeFET technology results in the lowest total energy. After those point, the opt. STT results in the lowest energy for both tasks. The difference in transition point between FeFET and STT for the two workloads is due to the fact that ALBERT has higher energy inferences since sentence classification is a particularly intensive task.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.22\textwidth]{figures/ResNet26-int.png}
    \includegraphics[width=0.22\textwidth]{figures/ALBERT-int.png}
    \caption{The eNVM storage solution (iso-capacity arrays provisioned per task, optimized for ReadEDP) that minimizes total energy consumption varies according to system wake-up frequency and DNN inference task; All solutions shown maintain application accuracy and a 1s latency per inference.}
    \label{fig:intermittent}
\end{figure}


\subsection{Write Buffering Could Change \\ Performance Comparison Landscape} 
\label{subsec:write-buf}

In conjunction with technology innovation to reduce write latency, adoption of a wider set of eNVMs in general-purpose computing contexts could be made possible by employing existing architectural techniques to mask poor write characteristics. For example, in an effort to extend memory lifetime and mask the performance impact of write access, a more performant technology (e.g., SRAM, or STT) could be employed as a write-buffer. For illustrative purposes, we consider a simple SRAM write cache that would hold write requests to the eNVM, write back to eNVM when the buffer is full, and allow in-place updates in the case of multiple writes to the same address before an update to eNVM. Rather than employ a costly and engineering-intensive cycle-accurate simulator to gauge the impact of provisioning a write buffer, \NAME~enables an analytical study under user-specified traffic patterns to narrow the space of eNVMs worthy of further simulation and design effort in this case. This approach guides the high-level questions regarding whether write-buffering could make a difference in enabling additional technologies for applications with significant write traffic, and, if so, how much benefit would need to be extracted using the write buffer?

Figure \ref{fig:write_buffer} shows the results for this study for the SPEC2017 and Facebook-Graph-BFS. In particular, we look at the effects of masking write latency and reducing write traffic on total memory latency and power. We observe that for Facebook-Graph-BFS, if the write traffic load is reduced, FeFET now becomes a comparable option, while  for SPEC2017, FeFET is not able to meet the application traffic load regardless of write masking techniques. STT and RRAM are still the optimal technology choices for SPEC2017.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/wbuff-latency.png}
    \caption{Masking write latency or reducing write traffic via introduction of a write buffering scheme enables a broader set of eNVM technologies in terms of performance, power, and memory lifetime.}
    \label{fig:write_buffer}
\end{figure}


%\subsubsection{eNVM Between LLC and Main Memory} 
%\label{subsec:new-mem-level}

%\textcolor{red}{Candidate to cut this subsubsection for space?}
%While Section \ref{subsec:llc} and much previous work explicitly considers eNVM storage solutions to replace LLC traffic, another promising use case for these technologies could lie in intermediate storage -- an on-chip, dense resource for a larger set of application data separate from main memory.
%As a proxy for the viability of this use case, we consider 64MB capacity eNVM memory arrays evaluated under traffic patterns to DRAM during SPEC CPU2017 workload execution.
%We observe \textcolor{red}{describe figure}


%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.48\textwidth]{figures/FigPowerLifetimeMain.jpg}
%    \caption{Several eNVM proposals hold promise as a storage solution between LLC and main memory for general purpose compute across SPEC CPU2017 benchmarks.}
%    \label{fig:new-mem-level}
%\end{figure}

==> device_driven_opps.tex <==
%\subsection{Circuit \& Device-Driven Opportunities} \label{subsec:device-driven}
%\textcolor{red}{Summarize promising pairings of technology to arch constraints and/or to applications, with optional ``what if" addenda (e.g., IF endurance of technology X improved by Y, it would become feasible for application Z.  Would be nice to have a collection of smaller takeaways in this vein)}

%Computer architects are typically reliant on which technologies are available and mature for consideration in system contexts.
%However, \NAME~empowers cross-stack co-design between architects and device designers. In this section we discuss some of the co-design opportunities unlocked by \NAME. By contextualizing and evaluating the higher-level implications of cell-level innovations as they emerge, one can identify what system-level opportunities are unlocked by that change. An example of this is demonstrated in Section \ref{subsubsec:bg_fefet}.
%Another opportunity is to relax certain cell-level parameters in order to better suit certain applications or system priorities, which is the focus of Section \ref{subsubsec:area_eff}. Finally we give an example of how \NAME~can be used to deduce which device-level characteristics are most limiting to the adoption of a given eNVM in a given system context. This is discussed in Section \ref{subsubsec:mlc}, and is clear guide for future device innovations and array-level optimizations.


\subsection{Alternative FeFET Fabrication Choices \\ Unlock Performant Solutions} \label{subsec:bg_fefet}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/FigBGfefet.png}
    \caption{Alternative FeFET Fabrication Choices Unlock Performant Solutions. Back-gated (BG) FeFETs now provide the highest density and lowest operating power for example graph processing benchmarks with SRAM-comparable performance and begin to close the performance gap between non-BG FeFET and other memory technologies across SPEC2017.}
    \label{fig:bg_fefet}
\end{figure}

Previous FeFET-based memory device characterization and modeling efforts have exhibited write pulses on the order of $100ns$-$1\mu s$.
However, alternative FeFET fabrication strategies in early development stages, such as back-gated FeFETs \cite{intel_beol}, offer compelling potential advancements in write latency ($10ns$ programming pulse) and projected endurance ($1e12$). As noted in Section \ref{subsec:graphs}, the primary limiting factor to FeFET-based memory in the context of graph processing was an inability to meet the application latency targets under higher write traffic. Thus, using the underlying cell properties of back-gated FeFETS reported in \cite{intel_beol}, we can rapidly re-examine the viability of FeFET-based memory and probe whether this change could make a difference in the viability of FeFET-based memory for graph processing.

Figure \ref{fig:bg_fefet} shows the total power and total memory latency of an 8MB memory array with back-gated FeFET-based (in yellow) compared to using previous FeFET standards (red, green) and SRAM (blue). We examine these metrics under a range of read and write traffic patterns which are inclusive of the graph benchmarks described in Section~\ref{subsec:graphs} and the SPEC benchmarks used in Section~\ref{subsec:llc}. Three different array organizations are tested which represent three different optimization targets: read latency, read energy, and read EDP. In addition to estimating total power and latency, we perform an underlying array-level characterization, which is shown in Figure \ref{fig:bg_fefet} on the right. From the array characterization, we observe that the back-gated FeFETs show a slight increase in read energy per access and slight decrease in storage density compared to prior state-of-the-art cells. However, we can observe that they enable comparable application latency to SRAM across a wide range of write traffic where previous FeFET versions fall short. Furthermore, back-gated FeFETs results in the lowest operating power over most of the range of read accesses per second, including for the example graph processing benchmark, Wikipedia--BFS8MB. 

Based on these observation, we can conclude that these back-gated FeFET memory arrays have started to close the performance gap between non-BG FeFET and other memory technologies (including SRAM). \NAME's ability both to quickly and efficiently gauge the impact of cell-level innovations and to match emerging device designs to compelling use cases can enable productive co-design collaborations in the future. This feedback loop is mutually beneficial in providing direct motivation for further development of a given cell proposal and encouraging system designers to integrate more energy-efficient, highly dense on-chip memory.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/FigAreaEff.png}
    \caption{Trading Area Efficiency for Increased Performance. Using \NAME, the data is filtered for the bolded technologies in the upper-right plot. Memories that exhibit lower area efficiency tend to result in low total memory latency across many traffic scenarios.}
    \label{fig:area_eff}
\end{figure}


\subsection{Trading Area Efficiency for Increased \\ Performance} \label{subsec:area_eff}

One theme we can highlight across the architecture-driven case studies from Section~\ref{sec:case_studies} is that the subset of characterized results that exhibit lower area efficiency (i.e., internal array architectures that do less amortization of periphery and sensing overhead) also tend to result in lower total memory latency across many traffic scenarios. This is perhaps counter-intuitive given the effort spent in the devices community to manufacture very small cell sizes. We also note that in Figure \ref{fig:area_eff}, where such design points are highlighted across the plots, that slight advantages in terms of energy-per-access (e.g., Opt. STT and PCM compared to FeFET) tend to correlate to large total power advantages in high-traffic scenarios. As such, pointing out to device designers the greater relative impact of reduced energy per access rather than decreased cell size could usher in a more productive, product-ready set of eNVM technologies. 
Additionally, we observe that reducing energy per write access for STT and RRAM would drastically improve their relative power advantage for data-intensive applications, even at a cost of relatively lower area efficiency or storage density.


\subsection{Multi-Level Programming Advantages \\Vary Per Technology} \label{subsec:mlc}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/FigMLC.png}
    \caption{Achievable storage density via multi-level programming varies per technology; here, we filter those memory solutions that don't provide acceptable application accuracy for ResNet18 inference after fault injection trials, and we note that MLC RRAM offers denser, more performant memory than SLC RRAM while meeting application accuracy, while MLC FeFET is only sufficiently reliable for larger cell sizes (pessimistic points). \textcolor{red}{Fixme, should this be filtered to just the SLC /MLC / RRAM / FeFET comparison?  Or is the context helpful?}}
    \label{fig:mlc}
\end{figure}

While programming multiple bits per memory cell is an important strategy for increasing storage density across many eNVM proposals, previous work has revealed that MLC eNVMs often exhibit significantly higher fault rates that must be carefully considered in conjunction with application resilience \cite{maxnvm}. \NAME~enables efficient and broad probing of reliability vs. storage density by providing an application-agnostic fault injection tool and templates for technology-specific fault modes, as discussed in Section~\ref{subsubsec:fault_modeling}.
To demonstrate, we evaluate the impact of density on application accuracy for image classification using ResNet18 under storage in SLC vs. 2-bit MLC across multiple technologies which provide MLC capabilities and for which there exists sufficient cell and circuit level modeling to produce detailed fault models. The density vs. reliability trade-off is distinct for each technology. For example, Figure \ref{fig:mlc} displays 8MB and 16MB characterized arrays for storing weights for ResNet18 inference, including 2-bit MLC RRAM and 2-bit MLC FeFET, filtered such that only those arrays meeting application latency requirements and acceptable image classification accuracy are included. Note that these results replicate previous efforts that indicate that image classification inference is robust to 2-bit MLC RRAM storage (of note, we also verified this accuracy finding for CTT-based memories with fault modeling details provided in \cite{maxnvm, dac_ctt}), while we show that MLC FeFET devices only exhibit acceptable accuracy for larger cell sizes (pessimistic cell assumptions). This is because smaller FeFET cells are more difficult to program reliably due to increased device-to-device variation, but we note that optimistic SLC FeFETs offer denser, more reliable storage than larger, MLC-programmed FeFET-based memories. 


%\subsection{Identifying Limiting Cell Characteristic \\ Per Technology}

%\textcolor{red}{How about a limit study for each technology vs. (1) cell size, (2) set/reset/write pulse and (3) set/reset/write energy, run NVSim for iso-capacity across opt targets, look at power/perf/area across \textbf{all} traffic ranges and have a per-technology set of takeaways.  In interest of time/space, let's start with two that will definitely have different trade-offs -- RRAM and STT ?}

==> tables/related.tex <==
\begin{table*}[b] \small \begin{center} {
\begin{tabular}{cl|l|l|l|l|l|l|}
\begin{tabular}{|l|l|l|l|l|l|l|} 
\hline
                                   & Design Knobs and~ Constraints & {[}] & ISSWC & MaxNVM & DeepNVM++ & This Work  \\ 
\hline
\multirow{5}{*}{Application-Level} & Data Resilience               &      &       & \checkmark      &           & X          \\ 
\cline{2-7}
                                   & Data Format                   &      &       & X      &           & X          \\ 
\cline{2-7}
                                   & Application Accuracy          &      &       & X      &           & X          \\ 
\cline{2-7}
                                   & Application Latency           &      &       & X      &           & X          \\ 
\cline{2-7}
                                   & Domain-Specific Proposal      &      &       & X      &           &            \\ 
\hline
\multirow{6}{*}{System-Level}      & Memory Fault Injection        &      &       & X      &           & X          \\ 
\cline{2-7}
                                   & GPU-Specific                  &      &       &        &           & X          \\ 
\cline{2-7}
                                   & CPU-Specific                  &      &       &        &           & X          \\ 
\cline{2-7}
                                   & Accelerator Architecture      &      &       & X      &           & X          \\ 
\cline{2-7}
                                   & System Area                   &      &       & X      &           & X          \\ 
\cline{2-7}
                                   & System Power                  &      &       & X      &           & X          \\ 
\hline
\multirow{5}{*}{Technology-Level}  & Device Size                   &      &       &        &           & X          \\ 
\cline{2-7}
                                   & Device Endurance              &      &       &        &           & X          \\ 
\cline{2-7}
                                   & Periphery Overhead            &      &       &        &           & X          \\ 
\cline{2-7}
                                   & Cell Fault Rate / Model       &      &       & X      &           & X          \\ 
\cline{2-7}
                                   & Data Retention                &      &       &        &           & X          \\
\hline
\end{tabular}

 %    ITRS [] &  &  & over9000 &  & 1776-1777 &  &  &  &  & & \\ \hline
%     IRDS \cite{ieee irds} &  & & over9000 &  &  &  &  &  & & &\\ \hline
%     Stanford thing[]&  &  &  &  &  &  &  &  & & &\\ \hline
%     NVSim []& x & x &  &  &  &  &  &  & & &\\ \hline
%     NVMain []& x & x &  &  &  &  &  &  & & &\\ \hline
%     DESTINEY []& x & x &  &  &  &  &  &  & & &\\ \hline
%     NeuroSim []&  &  &  &  &  &  &  &  & & &\\ \hline
 %    Papers that connect NVSIM/NVMAIN with arch sim. &  &  &  &  &  &  &  &  & & &\\ \hline
 %    Hankin et al IISWC [] & x &  &  &  &  &  &  & x & & &\\ \hline
%    DeepNVM++ [] & x &  &  &  &  &  &  & x & & &\\ \hline
 %    \bf this work & \bf x & \bf x & \bf x & \bf x & \bf x & \bf x & \bf x & \bf x & \bf x & \bf x & \bf x & \\
    %\end{tabular} 
    } \caption{Comprehensive comparison of available simulation and DSE tools related to eNVMs. Aggressive about why this work is both novel, timely, and necessary. Prove this will be the one stop shop for NVM related stuff (and memory in general?) \textcolor{red}{Very rough draft, but something like this?}} \label{Related Work} \end{center}
    \end{table*}
